Refining 3D Human Texture Estimation from a Single Image

Estimating 3D human texture from a single image is essential in graphics and vision. It requires learning a mapping function from input images of humans with diverse poses into the parametric (UV) space and reasonably hallucinating invisible parts. To achieve a high-quality 3D human texture estimation, we propose a framework that adaptively samples the input by a deformable convolution where offsets are learned via a deep neural network. Additionally, we describe a novel cycle consistency loss that improves view generalization. We further propose to train our framework with an uncertainty-based pixel-level image reconstruction loss, which enhances color fidelity. We compare our method against the state-of-the-art approaches and show significant qualitative and quantitative improvements.

==> 6_sup.tex <==

\begin{table*}[t]
\caption{Refinement Network based on Deformable Convs}
\label{tab:arch_all}
\centering
\renewcommand\tabcolsep{3pt}
\begin{tabular}{|l|cc|cc|cc|cc|}
\hline
& \multicolumn{2}{c}{SSIM \ \ \ $\Uparrow$} & \multicolumn{2}{|c}{LPIPS \ \ \ $\Downarrow$} & \multicolumn{2}{|c}{CosSim \ \ \ $\Uparrow$}  & \multicolumn{2}{|c|}{CosSim-R \ \ \ $\Uparrow$} \\
\hline
& SV & NV & SV & NV & SV & NV & SV & NV \\
\hline
Pretrained &  0.7422 & 0.6535 & 0.1154  & 0.2040 & 0.5747 & 0.4943 & 0.5422 & 0.4736\\
Batch size = 8 & 0.7371 & 0.6524 & 0.1180 & 0.2047 & 0.5763 & 0.4966 & 0.5437 & 0.4761 \\
Single View (252k) & 0.7706 & 0.6494 & 0.0963 & 0.2150 & 0.5823 & 0.4809  & 0.5496 & 0.4585 \\
\hline
v1.0.0 & 0.7447 & 0.6514 & 0.1124 & 0.2029 & 0.5759 & 0.4949 & 0.5432 & 0.4743 \\
v1.0.1 & 0.7373 & 0.641 & 0.116 & 0.2027 & 0.5753 & 0.4949 & 0.5423 & 0.4738 \\
v1.1.0 & 0.7679 & 0.6501 & 0.099 & 0.2108 & 0.5778 & 0.4842 & 0.5454 & 0.4625 \\
v1.1.1 & 0.7656 & 0.6505 & 0.098 & 0.2095 & 0.5804 & 0.4847 & 0.5487 & 0.4635 \\
\hline
v2.0.0 & 0.7445 & 0.6515 & 0.1124 & 0.2035 & 0.5759 & 0.4948 & 0.5433 & 0.4739 \\
v2.0.1 & 0.7427 & 0.6519 & 0.114 & 0.2035 & 0.5747 & 0.4943 & 0.5419 & 0.4731 \\
v2.1.0 & 0.7504 & 0.6534 & 0.1132 & 0.2077 & 0.5421 & 0.4712 & 0.5132 & 0.4509 \\
v2.1.1 & 0.7377 & 0.6514 & 0.1186 & 0.2033 & 0.573 & 0.4944 & 0.5388 & 0.4724 \\
v2.1.2 & 0.7444 & 0.6524 & 0.1131 & 0.2034 & 0.5765 & 0.4952 & 0.5437 & 0.4743 \\
v2.1.3 & 0.7260 & 0.6501 & 0.1256 & 0.2052 & 0.5477 & 0.4798 & 0.5155 & 0.4587 \\
v2.1.5 & 0.7454 & 0.6538 & 0.1137 & 0.204 & 0.5742 & 0.4943 & 0.541 & 0.4723 \\
v2.2.0 & 0.7536 & 0.6536 & 0.1089 & 0.2072 & 0.5483 & 0.4742 & 0.5196 & 0.4546 \\
v2.2.1 & 0.7385 & 0.6503 & 0.118 & 0.2043 & 0.5735 & 0.4943 & 0.5394 & 0.4726 \\
v2.2.2 & 0.7427 & 0.6516 & 0.115 & 0.2043 & 0.5752 & 0.4945 & 0.5423 & 0.4732 \\
\hline
v3.0.0 & 0.7428 & 0.6518 & 0.1151 & 0.2044 & 0.5762 & 0.4949 & 0.543 & 0.4736 \\
\hline
v4.0.0 & 0.7424 & 0.6526 & 0.1159 & 0.2039 & 0.5738 & 0.4939 & 0.5408 & 0.4728 \\
v4.0.1 & 0.7409 & 0.6509 & 0.1161 & 0.2044 & 0.5739 & 0.4934 & 0.5416 & 0.4731 \\
v4.1.0 & 0.7421 & 0.6521 & 0.1133 & 0.2051 & 0.5608 & 0.4845 & 0.5286 & 0.4635 \\
v4.1.1 & 0.7198 & 0.6504 & 0.131 & 0.2051 & 0.5648 & 0.4941 & 0.5281 & 0.4704 \\
v4.1.2 & 0.7408 & 0.6511 & 0.1153 & 0.2071 & 0.5651 & 0.4872 & 0.5323 & 0.4661 \\
\hline
\end{tabular}
\end{table*}

\begin{table*}[t]
\caption{Refinement Network - Mask Network}\label{tab:arch_maskall}
\centering
\renewcommand\tabcolsep{3pt}
\begin{tabular}{|l|cc|cc|cc|cc|}
\hline
& \multicolumn{2}{c}{SSIM \ \ \ $\Uparrow$} & \multicolumn{2}{|c}{LPIPS \ \ \ $\Downarrow$} & \multicolumn{2}{|c}{CosSim \ \ \ $\Uparrow$}  & \multicolumn{2}{|c|}{CosSim-R \ \ \ $\Uparrow$} \\
\hline
& SV & NV & SV & NV & SV & NV & SV & NV \\
\hline
Pretrained &  0.7422 & 0.6535 & 0.1154  & 0.2040 & 0.5747 & 0.4943 & 0.5422 & 0.4736\\
Batch size = 8 & 0.7371 & 0.6524 & 0.1180 & 0.2047 & 0.5763 & 0.4966 & 0.5437 & 0.4761 \\
\hline
MN v1 & 0.756 & 0.654 & 0.1053 & 0.202 & 0.5813 & 0.4802 & 0.5481 & 0.4767 \\ 
RN v2.2.2 & 0.7427 & 0.6516 & 0.115 & 0.2043 & 0.5752 & 0.4945 & 0.5423 & 0.4732 \\
\hline
v1.0-2.2.2-1 & 0.7481 & 0.6537 & 0.1122 & 0.2041 & 0.5734 & 0.4938 & 0.5407 & 0.4727 \\
v1.1-2.2.2-1 & 0.7561 & 0.6547 & 0.1071 & 0.203 & 0.5815 & 0.4978 & 0.5495 & 0.4773 \\
v1.0-2.1.2-1 & 0.7522 & 0.6539 & 0.1092 & 0.2032 & 0.575 & 0.4937 & 0.5431 & 0.4732 \\
v1.1-2.1.2-1 & 0.765 & 0.6582 & 0.1041 & 0.2011 & 0.578 & 0.4958 & 0.5452 & 0.4753 \\
\hline
\end{tabular}
\end{table*}

\begin{table*}[t]
\caption{Cycle Network}\label{tab:cycle}

\centering
\renewcommand\tabcolsep{3pt}
\begin{tabular}{|l|cc|cc|cc|cc|}
\hline
& \multicolumn{2}{c}{SSIM \ \ \ $\Uparrow$} & \multicolumn{2}{|c}{LPIPS \ \ \ $\Downarrow$} & \multicolumn{2}{|c}{CosSim \ \ \ $\Uparrow$} & \multicolumn{2}{|c|}{CosSim-R \ \ \ $\Uparrow$} \\
\hline
& SV & NV & SV & NV & SV & NV & SV & NV \\
\hline
Pretrained &  0.7422 & 0.6535 & 0.1154  & 0.2040 & 0.5747 & 0.4943 & 0.5422 & 0.4736\\
Batch size = 8 & 0.7371 & 0.6524 & 0.1180 & 0.2047 & 0.5763 & 0.4966 & 0.5437 & 0.4761 \\
\hline
L2 loss btw. UV-Maps & 0.7448 & 0.6503 & 0.1107 & 0.2027 & 0.5837 & 0.4968 & 0.5502 & 0.4761 \\ 
VGG loss btw. UV-Maps & 0.7042 & 0.6485 & 0.1342 & 0.2022 & 0.5643 & 0.4968 & 0.5259 & 0.4725 \\
Batch 4 L2 loss btw. UV-RGBs & 0.7436 & 0.6523 & 0.1118 & 0.2030 & 0.5818 & 0.4993 & 0.5487 & 0.4768 \\
Batch 8 L2 loss btw. UV-RGBs & 0.7457 & 0.6515 & 0.1110 & 0.2033 & 0.5826 & 0.4989 & 0.5493 & 0.4771 \\
Batch 4 L2 loss btw. UV-Maps and UV-RGBs & 0.7445 & 0.6516 & 0.1122 & 0.2042 & 0.5829 & 0.4987 & 0.5497 & 0.4773 \\
Batch 8 L2 loss btw. UV-Maps and UV-RGBs & 0.7451 & 0.6500 & 0.1120 & 0.2040 & 0.5829 & 0.4988 & 0.5491 & 0.4762 \\

\hline
\end{tabular}
\end{table*}

\begin{table*}[t]
\caption{Refinement Network - Mask Network - Cycle}\label{tab:arch_maskall2}
\centering
\renewcommand\tabcolsep{3pt}
\begin{tabular}{|l|cc|cc|cc|cc|}
\hline
& \multicolumn{2}{c}{SSIM \ \ \ $\Uparrow$} & \multicolumn{2}{|c}{LPIPS \ \ \ $\Downarrow$} & \multicolumn{2}{|c}{CosSim \ \ \ $\Uparrow$}  & \multicolumn{2}{|c|}{CosSim-R \ \ \ $\Uparrow$} \\
\hline
& SV & NV & SV & NV & SV & NV & SV & NV \\
\hline
Pretrained &  0.7422 & 0.6535 & 0.1154  & 0.2040 & 0.5747 & 0.4943 & 0.5422 & 0.4736\\
Batch size = 8 & 0.7371 & 0.6524 & 0.1180 & 0.2047 & 0.5763 & 0.4966 & 0.5437 & 0.4761 \\
\hline
Baseline + RN + URL - v1.1-2.1.2-1 (1) & 0.765 & 0.6582 & 0.1041 & 0.2011 & 0.578 & 0.4958 & 0.5452 & 0.4753 \\
\hline
(1) + UVRGB based on Texformer & 0.75 & 0.6532 & 0.1139 & 0.2055 & 0.5767 & 0.4948 & 0.5445 & 0.4723 \\
(1) + UVRGB based on RN & 0.7489 & 0.6562 & 0.114 & 0.2042 & 0.5741 & 0.4944 & 0.5409 & 0.4715 \\
(1) + UVRGB + UVMAP based on RN & 0.7477 & 0.653 & 0.1152 & 0.2054 & 0.5775 & 0.4964 & 0.5442 & 0.4744 \\
\hline
\end{tabular}
\end{table*}

% \begin{table*}
% \centering
% \renewcommand\tabcolsep{3pt}
% \begin{tabular}{l|cc|cc|cc|cc|}
% & \multicolumn{2}{c}{SSIM} $\Uparrow$ & \multicolumn{2}{c}{LPIPS} $\Downarrow$  & \multicolumn{2}{c}{CosSim $\Uparrow$}  & \multicolumn{2}{c}{CosSim-R} $\Uparrow$ \\
% \hline
% & SV & MV & SV & MV & SV & MV & SV & MV \\
% \hline
% Pretrained &  0.7422 & 0.6535 & 0.1154  & 0.2040 & 0.5747 & 0.4943 & 0.5422 & 0.4736\\
% Batch size = 8 & 0.7371 & 0.6524 & 0.1180 & 0.2047 & 0.5763 & 0.4966 & 0.5437 & 0.4761 \\
% \hline
%  (Batch size = 4)\footnotemark  & 0.7357 & 0.6505 & 0.1123 & 0.2062 & 0.5789 & 0.4950 & 0.5475 & 0.4735 \\
%  + pretrained texformer\footnotemark  & 0.7355 & 0.6492 & 0.1133 & 0.2046 &0.5806 & 0.4970 & 0.5491 & 0.4768\\

% \hline
% Texformer Style  - v2  & 0.7389& 0.6522 & 0.1121 & 0.2043 & 0.5807 & 0.4972 & 0.5497 & 0.4764 \\
% Texformer Style  - v3  & 0.7372& 0.6526 & 0.1142 & 0.2058 & 0.5804 & 0.4970 & 0.5485 & 0.4763 \\
% \hline
% Small Unet Without Att & 0.7394 & 0.6520 & 0.1108 & 0.2040 & 0.5797 & 0.4965 & 0.5490 & 0.4762 \\
% Small Unet with Att &0.7369 & 0.6504 & 0.1131 & 0.2050 & 0.5799 & 0.4964 & 0.5488 & 0.4764 \\
% Unet Att- First last  & 0.7182 & 0.6516 & 0.1278 & 0.2039 & 0.5696 & 0.4970 & 0.5344 & 0.4752\\
% Unet Att- First last-v2 & 0.7371 & 0.6509 & 0.1126 & 0.2048 & 0.5803 & 0.4968 & 0.5494 & 0.4759 \\
% Unet Att-First last-v3  & 0.7379 & 0.6512 & 0.1132 & 0.2048 & 0.5803 & 0.4965 & 0.5489 & 0.4757 \\
% \end{tabular}
% \end{table*}





\begin{table*}[t]
\caption{Mask Network Models}\label{tab:arch_mall1}
\centering
\renewcommand\tabcolsep{2pt}
\begin{tabular}{|l|cc|cc|cc|cc|}
\hline
& \multicolumn{2}{c}{SSIM \ \ \ $\Uparrow$} & \multicolumn{2}{|c}{LPIPS \ \ \ $\Downarrow$} & \multicolumn{2}{|c}{CosSim \ \ \ $\Uparrow$}  & \multicolumn{2}{|c|}{CosSim-R \ \ \ $\Uparrow$} \\
\hline
& SV & MV & SV & MV & SV & MV & SV & MV \\
\hline
Pretrained &  0.7422 & 0.6535 & 0.1154  & 0.2040 & 0.5747 & 0.4943 & 0.5422 & 0.4736\\
\hline
(1) + Pretrained, SV & 0.7504 & 0.6529 & 0.1121 & 0.2046 & 0.5778 & 0.4963 & 0.5455 & 0.4759 \\
(2), Multi-view & 0.7473 & 0.6620 & 0.1132 & 0.2004 & 0.57 & 0.4941 & 0.5382 & 0.4734\\
(2) + Foreground Mask (3), SV & 0.7412 & 0.6512 & 0.1141 & 0.2043 & 0.5725 & 0.4947 & 0.5394 & 0.4741 \\
(3), Multi-view & 0.7381 & 0.6557 & 0.1178 & 0.2025 & 0.5667 & 0.4924 & 0.5340 & 0.4706 \\
\hline
\parbox[c]{5.05cm}{Mask Network Input Tuning v1 - (1), Input image + 1 Seg, SV} & \multirow{1}{*}{0.756} & \multirow{1}{*}{0.654} & \multirow{1}{*}{0.1053} & \multirow{1}{*}{0.202} & \multirow{1}{*}{0.5813} & \multirow{1}{*}{0.4802} & \multirow{1}{*}{0.5481} & \multirow{1}{*}{0.4767} \\
\hline
\end{tabular}
\end{table*}



\begin{table*}[t]
\caption{Ablation Study}\label{tab:full_abl}

\centering
\renewcommand\tabcolsep{3pt}
\begin{tabular}{|l|cc|cc|cc|cc|}
\hline
& \multicolumn{2}{c}{SSIM \ \ \ $\Uparrow$} & \multicolumn{2}{|c}{LPIPS \ \ \ $\Downarrow$} & \multicolumn{2}{|c}{CosSim \ \ \ $\Uparrow$} & \multicolumn{2}{|c|}{CosSim-R \ \ \ $\Uparrow$} \\
\hline
& SV & NV & SV & NV & SV & NV & SV & NV \\
\hline
BL (Baseline) &  0.7422 & 0.6535 & 0.1154  & 0.2040 & 0.5747 & 0.4943 & 0.5422 & 0.4736\\
\hline
BL + Refine  & 0.7444 & 0.6524 & 0.1131 & 0.2034 & 0.5765 & 0.4952 & 0.5437 & 0.4743 \\
BL + Cycle & 0.7448 & 0.6503 & 0.1107 & 0.2027 & 0.5837 & 0.4968 & 0.5502 & 0.4761 \\ 
BL + URL & 0.7560 & 0.6540 & 0.1053 & 0.2020 & 0.5813 & 0.4802 & 0.5481 & 0.4767 \\
BL + Refine + URL 140k & 0.7650 & 0.6582 & 0.1041 & 0.2011 & 0.5780 & 0.4958 & 0.5452 & 0.4753 \\
BL + Refine + URL 175k & 0.7609 & 0.6552 & 0.107 & 0.2033 & 0.5785 & 0.4962 & 0.5456 & 0.4735 \\
BL + Refine + URL 210k &  0.7585 & 0.6547 & 0.1076 & 0.2027 & 0.5798 & 0.4971 & 0.5466 & 0.475 \\
BL + Refine + Cycle + URL 78.75k & 0.7594 & 0.6546 & 0.108 & 0.2039 & 0.5797 & 0.497 & 0.5469 & 0.4745 \\
BL + Refine + Cycle + URL 87.5k & 0.7535 & 0.6547 & 0.1104 & 0.2035 & 0.5806 & 0.4978 & 0.5472 & 0.4747 \\
\hline
\end{tabular}
\end{table*}
